Promoting Robustness of Randomized Smoothing: Two Cost-Effective Approaches

Randomized smoothing has recently attracted attentions in the field of adversarial robustness to provide provable robustness guarantees on smoothed neural network classifiers. However, existing works show that vanilla randomized smoothing usually does not provide good robustness performance and often requires (re)training techniques on the base classifier in order to boost the robustness of the resulting smoothed classifier. In this work, we propose two cost-effective approaches to boost the robustness of randomized smoothing while preserving its clean performance. The first approach introduces a new robust training method AdvMacerwhich combines adversarial training and robustness certification maximization for randomized smoothing. We show that AdvMacer can improve the robustness performance of randomized smoothing classifiers compared to SOTA baselines, while being 3x faster to train than MACER baseline. The second approach introduces a post-processing method EsbRS which greatly improves the robustness certificate based on building model ensembles. We explore different aspects of model ensembles that has not been studied by prior works and propose a novel design methodology to further improve robustness of the ensemble based on our theoretical analysis.

==> algorithms/alg_and_figure.tex <==
\begin{tabular}{cc}
\raisebox{0.1cm}{\begin{minipage}{.58\textwidth}
\includegraphics[width=\textwidth]{figures/ensemble_new.png}
\captionof{figure}{The plot of ACR against different number of component models in \EsbRs{} on Cifar-10 with $\sigma=0.50$. Mixed-model ensemble uses $m$ \ourmethod models and $n$ SmoothAdv models, where $m$ and $n$ are given the plot.}
\label{fig:ensemble}
\end{minipage}} &
\begin{minipage}{.42\textwidth}
\input{algorithms/alg_esb-max}
\end{minipage}
\end{tabular}

==> algorithms/alg_distillation.tex <==
\begin{algorithm}[th!]
\caption{Knowledge distillation}
\label{alg:distillation}
\begin{algorithmic}
   \STATE {\bfseries Input:} training data $\hat p_{\text{data}}$, a teacher model $H$, a loss function $L$ chosen from MSE loss $L_{\text{MSE}}$, and ReLU loss $L_{\text{ReLU}}$ as defined in \eqref{eq:relu}, number of noise vector $m$, noise level $\sigma$, boolean variable to indicate whether original cross-entropy loss is included
   \FOR{each iteration}
    \STATE 1) Sample a mini-batch $(x_1, y_1),\dots,(x_n,y_n)\sim\hat p_{\text{data}}$
    \STATE 2) For each $(x_i, y_i)$, draw $m$ i.i.d. Gaussian samples $x_{i1},\dots,x_{im}$ from $\mathcal{N}(x_i,\sigma^2I)$
    \STATE 3) Estimate the expectations:
    \begin{align*}
        \hat z_\theta(x_i) &\gets \frac1m\sum_{k=1}^mF_\theta(x_{ik}), \text{ for } i=1,\dots, n\\
        \hat H(x_i) &\gets \frac1m\sum_{k=1}^mH(x_{ik}), \text{ for } i=1,\dots, n
    \end{align*}
    \STATE 4) Compute the loss: 
                $L=\frac1n\sum_{i=1}^n L(\hat z_\theta(x_i), \hat H(x_i))$
    \IF{include cross-entropy loss}
        \STATE Update the loss:
        $L \gets L + \frac1n\sum_{i=1}^n\log\hat z_\theta(x_i)_{y_i}$
    \ENDIF
    \ENDFOR   
    \STATE {\bfseries Output:} model parameters $\theta$
\end{algorithmic}
\end{algorithm}

==> algorithms/alg_esb-max.tex <==
\begin{algorithm}[H]
\caption{\EsbRs{-}max}
\label{alg:esb-max}
\begin{algorithmic}
   \State {\bfseries Input:} query point $x_0$, trained component models $f^1,\dots,f^k$, noise level $\sigma$, number of Gaussian samples for estimation $n_0$
   \State{\bfseries Output:} Weights $w_1,\dots,w_k$
   \For{$l=1,\dots,k$}
    \State 1) Draw $n$ samples  $\delta_1,\dots,\delta_{n_0}\sim\mathcal{N}(0, \sigma^2I)$ and compute $n_0$ predicted labels $f^l(x_0+\delta_1), \dots, f^l(x_0+\delta_{n_0}).$
    \State 2) Compute the majority vote: $c^l=\max_{i\in[C]}|\{j: f^l(x_0+\delta_j)=i\}|$
    \EndFor
    \State 3) Select the best classifier $j$ with largest majority vote: $j\in\argmax_{l=1,\dots,k}c^l$.
    \State 4) Set $w_j=1$ and $w_l=0$ for $l\neq j$.
\end{algorithmic}
\end{algorithm}

==> algorithms/alg_esb-max_correct.tex <==
\begin{algorithm}[H]
\caption{\EsbRs{-}max}
\label{alg:esb-max-correct}
\begin{algorithmic}
   \State {\bfseries Input:} query point $x$, Gaussian noise $\delta$, trained component models $f^1,\dots,f^k$, noise level $\sigma$, number of Gaussian samples for estimation $n_0$
   \State{\bfseries Output:} Weights $w_1(x+\delta),\dots,w_k(x+\delta)$
   \For{$l=1,\dots,k$}
    \State 1) Draw $n_0$ samples  $\epsilon_1,\dots,\epsilon_{n_0}\sim\mathcal{N}(0, \sigma^2I)$ and compute $n_0$ predicted labels $f^l(x+\delta+\epsilon_1), \dots, f^l(x+\delta+\epsilon_{n_0}).$
    \State 2) Compute the majority vote: $c^l=\max_{i\in[C]}|\{j: f^l(x+\delta+\epsilon_j)=i\}|$
    \EndFor
    \State 3) Select the best classifier $j$ with largest majority vote: $j\in\argmax_{l=1,\dots,k}c^l$.
    \State 4) Set $w_j=1$ and $w_l=0$ for $l\neq j$.
\end{algorithmic}
\end{algorithm}

==> algorithms/alg_wt_ensemble.tex <==
% \begin{algorithm}[th!]
% \caption{Optimal weights of ensemble with 2 models. The function \textbf{ComputeWeight} will return the optimal weights}
% \label{alg:wt_ensemble}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} two base models $F^1,F^2$, number of Gaussian noise $n$, number of perturbed models $m$, noise level $\sigma$, proportion of the parameters to perturb $t$, standard deviation of perturbation on parameters $\tilde\sigma$, query point $x$, target label $y$
%   \STATE{\bfseries function} PerturbModel($F^1,F^2,m,t,\tilde\sigma$):
%   \begin{ALC@g}
%     \FOR {$l=1,2$}
%       \FOR{each $j=1,\dots,m$}
%         \FOR {each parameter $\theta$ in $F^l$}
%             \STATE Draw a Bernoulli variable $X$ from $\text{Bernoulli}(t)$
%             \IF{$X=1$} 
%             \STATE Draw $\delta\sim\mathcal{N}(0,\tilde\sigma^2)$ and update $\theta\gets\theta+\delta$
%             \ENDIF
%         \ENDFOR
%         \STATE Store perturbed model $\hat F^{l}_j$
%         \ENDFOR
%         \ENDFOR
%         \STATE {\bfseries Output:} perturbed models $\hat F^1_1,\dots,F^1_m$ and $\hat F^2_1,\dots,\hat F^2_m$.
%     \end{ALC@g}
%     \STATE
%     \STATE{\bfseries function} Estimation([$\hat F^1_1,\dots,F^1_m$], [$\hat F^2_1,\dots,\hat F^2_m$], $\sigma,n,x,y$):
%     \begin{ALC@g}
%         \STATE Draw $n$ i.i.d. noisy samples from $\mathcal{N}(x,\sigma^2I)$ and denote them by $x_1,\dots,x_n$
%         \FOR{$l=1,2$}
%         \FOR{$i=1,\dots,m$}
%             \FOR{$j=1,\dots,n$}
%                 \STATE Compute $z^{l,(i-1)n+j}\gets\hat F^l_i(x_j)_y\mathbf{1}-\hat F^l_i(x_j)$, where $\mathbf{1}=[1,1,\dots,1]^\top$ is the vector of all 1's.
%             \ENDFOR
%         \ENDFOR
%         \ENDFOR
%         \STATE{\bfseries Output:} estimates of logits $z^{l,j}$ for $l=1,2$ and $j=1,\dots,mn$
%     \end{ALC@g}
%     \STATE
%     \STATE{\bfseries function} ComputeWeight($F^1,F^2,\sigma,\tilde\sigma,n,m,t,x,y$):
%     \begin{ALC@g}
%         \STATE 1) $[\hat F^1_1,\dots,F^1_m]$, $[\hat F^2_1,\dots,\hat F^2_m]$ $\gets$ PerturbModel($F^1,F^2,m,t,\tilde\sigma$)
%         \STATE 2) $z^{l,j}\gets$ Estimation([$\hat F^1_1,\dots,F^1_m$], [$\hat F^2_1,\dots,\hat F^2_m$], $\sigma,n,x,y$) for $l=1,2$ and $j=1,\dots,m$
%         \STATE 3) Compute $\bar z^l\gets\frac1{mn}\sum_{j=1}^{mn}z^{l,j}$ for $l=1,2$ and $a_i\gets\min\{\bar z^1_i,\bar z^2_i\}^{-2}$ for $i=1,\dots,c$
%         \STATE 4) Compute 
%                  $$   b_i\gets\frac1{mn}\sum_{j=1}^{mn}(z^{1,j}-\bar z^{1})(z^{1,j}-\bar z^{1})^\top_{ii},~
%                     c_i\gets\frac2{mn}\sum_{j=1}^{mn}(z^{1,j}-\bar z^{1})(z^{2,j}-\bar z^{2})^\top_{ii},~
%                     d_i\gets\frac1{mn}\sum_{j=1}^{mn}(z^{2,j}-\bar z^{2})(z^{2,j}-\bar z^{2})^\top_{ii},$$
%         \STATE 5) Compute $$ A=\sum_{i=2}^ca_i(b_i+c_i+d_i),\quad
%                 B=\sum_{i=2}^c -a_i(c_i+2d_i),\quad
%                 C=\sum_{i=2}^ca_id_i.$$
%         \IF{$A>0$ and $0\leq-\frac{B}{2A}\leq1$}
%         \STATE $w_1\gets-\frac{B}{2A}$ and $w_2\gets1+\frac{B}{2A}$
%         \ELSE
%         \STATE $w_1\gets0,w_2\gets1$ if $A+B>0$ else $w_1\gets1,w_2\gets0$
%         \ENDIF
%         \STATE{\bfseries Output:} $w_1,w_2$
%     \end{ALC@g}
% \end{algorithmic}
% \end{algorithm}

\algdef{SE}[SUBALG]{Indent}{EndIndent}{}{\algorithmicend\ }%
\algtext*{Indent}
\algtext*{EndIndent}

\begin{algorithm}[th!]
\caption{Optimal weights of ensemble with 2 models. The function \textbf{ComputeWeight} will return the optimal weights}
\label{alg:wt_ensemble}
\begin{algorithmic}
   \State {\bfseries Input:} two base models $F^1,F^2$, number of Gaussian noise $n$, number of perturbed models $m$, noise level $\sigma$, proportion of the parameters to perturb $t$, standard deviation of perturbation on parameters $\tilde\sigma$, query point $x$, target label $y$
   \State{\bfseries function} PerturbModel($F^1,F^2,m,t,\tilde\sigma$):
   \Indent
    \For {$l=1,2$}
       \For{each $j=1,\dots,m$}
        \For {each parameter $\theta$ in $F^l$}
            \State Draw a Bernoulli variable $X$ from $\text{Bernoulli}(t)$
            \If {$X=1$} 
            \State Draw $\delta\sim\mathcal{N}(0,\tilde\sigma^2)$ and update $\theta\gets\theta+\delta$
            \EndIf
        \EndFor
        \State Store perturbed model $\hat F^{l}_j$
        \EndFor
        \EndFor
        \State {\bfseries Output:} perturbed models $\hat F^1_1,\dots,F^1_m$ and $\hat F^2_1,\dots,\hat F^2_m$.
    \EndIndent
    \State
    \State{\bfseries function} Estimation([$\hat F^1_1,\dots,F^1_m$], [$\hat F^2_1,\dots,\hat F^2_m$], $\sigma,n,x,y$):
    \Indent
        \State Draw $n$ i.i.d. noisy samples from $\mathcal{N}(x,\sigma^2I)$ and denote them by $x_1,\dots,x_n$
        \For{}{$l=1,2$}
        \For{$i=1,\dots,m$}
            \For{$j=1,\dots,n$}
                \State Compute $z^{l,(i-1)n+j}\gets\hat F^l_i(x_j)_y\mathbf{1}-\hat F^l_i(x_j)$, where $\mathbf{1}=[1,1,\dots,1]^\top$ is the vector of all 1's.
            \EndFor
        \EndFor
        \EndFor
        \State{\bfseries Output:} estimates of logits $z^{l,j}$ for $l=1,2$ and $j=1,\dots,mn$
    \EndIndent
    \State
    \State{\bfseries function} ComputeWeight($F^1,F^2,\sigma,\tilde\sigma,n,m,t,x,y$):
    \Indent
        \State 1) $[\hat F^1_1,\dots,F^1_m]$, $[\hat F^2_1,\dots,\hat F^2_m]$ $\gets$ PerturbModel($F^1,F^2,m,t,\tilde\sigma$)
        \State 2) $z^{l,j}\gets$ Estimation([$\hat F^1_1,\dots,F^1_m$], [$\hat F^2_1,\dots,\hat F^2_m$], $\sigma,n,x,y$) for $l=1,2$ and $j=1,\dots,m$
        \State 3) Compute $\bar z^l\gets\frac1{mn}\sum_{j=1}^{mn}z^{l,j}$ for $l=1,2$ and $a_i\gets\min\{\bar z^1_i,\bar z^2_i\}^{-2}$ for $i=1,\dots,c$
        \State 4) Compute 
                 $$   b_i\gets\frac1{mn}\sum_{j=1}^{mn}(z^{1,j}-\bar z^{1})(z^{1,j}-\bar z^{1})^\top_{ii},~
                    c_i\gets\frac2{mn}\sum_{j=1}^{mn}(z^{1,j}-\bar z^{1})(z^{2,j}-\bar z^{2})^\top_{ii},~
                    d_i\gets\frac1{mn}\sum_{j=1}^{mn}(z^{2,j}-\bar z^{2})(z^{2,j}-\bar z^{2})^\top_{ii},$$
        \State 5) Compute $$ A=\sum_{i=2}^ca_i(b_i+c_i+d_i),\quad
                B=\sum_{i=2}^c -a_i(c_i+2d_i),\quad
                C=\sum_{i=2}^ca_id_i.$$
        \If{$A>0$ and $0\leq-\frac{B}{2A}\leq1$}
        \State $w_1\gets-\frac{B}{2A}$ and $w_2\gets1+\frac{B}{2A}$
        \Else
        \State $w_1\gets0,w_2\gets1$ if $A+B>0$ else $w_1\gets1,w_2\gets0$
        \EndIf
        \State{\bfseries Output:} $w_1,w_2$
    \EndIndent
\end{algorithmic}
\end{algorithm}


==> tables/table_cifar10.tex <==
\begin{table*}[t]
\caption{Cifar-10: ACR of different models on the first 500 test images of Cifar-10 with varing $\sigma$. Clean accuracy is reported in parenthesis. Reported models include SmoothAdv, MACER, \ourmethod, \EsbRs{}. $N=100,000$ samples are used in certification unless otherwise specified.}
\label{table_cifar10}
\vskip 0.15in
\begin{center}
\begin{small}
\scalebox{0.75}{
\begin{tabular}{llcccc}
\toprule
& Methods & $\sigma=0.25$ & $\sigma=0.5$ & $\sigma=1.0$ & Ensemble?\\
\midrule
\multirow{2}{4em}{\centering Baselines}
&SmoothAdv & 0.541 (74.2\%) & 0.735 (56.4\%) & 0.758 (45.8\%) & $\times$\\
&MACER &	0.518 (79.4\%) & 0.682 (63.4\%) & 0.768 (42.4\%)& $\times$\\
\midrule
\multirow{8}{4em}{\centering Ours}
&\ourmethod & \textbf{0.554 (76.0\%)} & \textbf{0.742 (58.4\%)} & \textbf{0.794 (47.6\%)}& $\times$\\
&\EsbRs{-}\ourmethod$\times3$ & \textbf{0.583} (76.4\%) & 0.772 (58.8\%)& 0.805 (47.6\%) & $\surd$\\
&\EsbRs{-}SmoothAdv$\times3$ & 0.567 (76.6\%) &0.777 (58.4\%) & 0.801 (46.6\%) & $\surd$\\
&\EsbRs{-}\ourmethod$\times$1+SmoothAdv$\times$2 & 0.572 (77.2\%) & \textbf{0.783} (59.4\%) & \textbf{0.810} (47.2\%) & $\surd$\\
&\EsbRs{-}\ourmethod$\times$2+MACER$\times$1 & 0.568 (79.8\%) & 0.728 (63.6\%) & 0.801 (42.8\%)& $\surd$\\
&\EsbRs{-}\ourmethod$\times$1+MACER$\times$2 & 0.570 (80.4\%) & 0.723 (65.0\%) & 0.760 (44.0\%)& $\surd$\\
&\EsbRs{-}\ourmethod$\times3$ with $N/3$ & 0.550 (76.4\%) & 0.736 (58.8\%) & 0.785 (47.4\%)& $\surd$\\
&SmoothAdv with $3N$ &0.568 (74.6\%) & 0.761 (56.8\%) & 0.771 (45.6\%)& $\times$\\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}



==> tables/table_distillation.tex <==
\begin{table}[ht]
\caption{Knowledge distillation. ACR and clean accuracy of different student models on the first 500 test images of Cifar-10 with $\sigma=0.25$. For comparison, the performance of component model (\ourmethod) and teacher (\ourmethod$\times3$) is also reported.}
\label{table_distillation}
\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc} 
\begin{tabular}{lccr}
\toprule
Model & Trained from & Accuracy & ACR\\
\midrule
\ourmethod & scratch & 0.760 & 0.554\\
\ourmethod$\times3$ & scratch & 0.764 & 0.583\\
Student with $L_{\text{MSE}}$ & scratch & 0.660 & 0.357\\
Student with $L_{\text{ReLU}}$ & scratch & 0.782 & 0.489\\
Student with $L_{\text{ReLU}}+L_{\text{CE}}$ & scratch & 0.794 & 0.454\\
Student with $L_{\text{ReLU}}+L_{\text{CE}}$ & pretrained \ourmethod & \textbf{0.810} & \textbf{0.508}\\ 
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\end{table}

==> tables/table_efficiency.tex <==
\begin{table*}[t]
\caption{Efficiency comparison of \ourmethod and MACER when $\sigma=0.25$.}
\label{table_acr_plot}
\vskip 0.15in
\begin{center}
\begin{small}
\scalebox{1}{
\begin{tabular}{ccccccc}
\toprule
Epochs & 25 & 50 & 75 & 100 & 125 & 150\\
\midrule
MACER & 0.165 & 0.337 & 0.370 & 0.397 & 0.460 & 0.497\\
\ourmethod & 0.457 &  0.471 & 0.530 & 0.530 & 0.537 & 0.554\\
ACR Improvement \\
\bottomrule
\end{tabular}
}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> tables/table_ensemble456.tex <==
\begin{table}[t]
\caption{The performance of different number of ensemble macer-ADV models on the first 500 test images of Cifar10.}
\label{table_ensemble456}
\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc} 
\begin{tabular}{lcr}
\toprule
Ensemble \# & Accuracy & ACR\\
\midrule
1 & 76\% & 0.554\\
2 & 76\% & 0.572\\
3 & 76.4\% & 0.583\\
4 & 76.6\% & 0.590\\
5 & 77.4\% & 0.590\\
6 & 77.6\% & 0.594\\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\end{table}

==> tables/table_ensemble_num.tex <==
\begin{table}[h!]
\caption{Component models in mixed ensemble experiment in \cref{fig:ensemble}. The mixed ensemble with totally $N$ component models uses $m$ \ourmethod and $n$ SmoothAdv models. $m$ and $n$ are given as follows.}
\label{table_ensemble_num}
\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc} 
\begin{tabular}{lcr}
\toprule
N & m & n\\
\midrule
1 & 1 & 0\\
2 & 1 & 1\\
3 & 1 & 2\\
4 & 2 & 2\\
5 & 3 & 2\\
6 & 3 & 3\\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\end{table}

==> tables/table_imagenet_esb.tex <==
\begin{table}[t]
% \caption{Weighted ensemble. ACR and clean accuracy on 500 test images of Cifar-10 with $\sigma=0.25$. All certification has parameters $N_0=100,N=100,000,\alpha=0.001$. \EsbRs{-}max is computed from \cref{alg:esb-max} with \ourmethod models and $n$ used in estimation are specified in parenthesis. }
\caption{Performance of ensemble of two \ourmethod on ImageNet dataset. $n_0$ is the number of samples used in \cref{alg:esb-max}. The certification is run with 4 NVIDIA V100 GPUs.}
\label{table_wt_ensemble}
\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc} 
\scalebox{0.8}{
\begin{tabular}{lcccc}
\toprule
Model & Accuracy & ACR & Certificate Time & Ensemble?\\
\midrule
\ourmethod & 0.639 & 0.537 & 23.9s & $\times$\\
Avg weight \EsbRs{} & 0.634 & 0.541 & 47.7s & $\surd$\\
MME \cite{yang2021certified} & 0.634 & 0.537 & 95.2s & $\surd$\\
% Optimal weight \EsbRs{} & \textbf{0.766} & \textbf{0.576} & 26.3\\
% \EsbRs{-}max ($n_0=10^2$)  & \textbf{0.650} & \textbf{0.565} & 24.1s & $\surd$\\
% \EsbRs{-}max ($n_0=10^4$)  & \textbf{0.766} & \textbf{0.597} & 10.8s & $\surd$\\
\bottomrule
\end{tabular}
}
%\end{sc}
\end{small}
\end{center}
\end{table}

==> tables/table_miniimagenet.tex <==
\begin{table*}[t]
\caption{Mini-ImageNet: ACR of different models on the first 500 test images of Mini-ImageNet with varing $\sigma$. Clean accuracy is reported in parenthesis. Reported models include SmoothAdv and \ourmethod.}
\label{table_main}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{cccc}
\toprule
Models & $\sigma=0.25$ & $\sigma=0.5$ & $\sigma=1.0$\\
\midrule
SmoothAdv~\cite{salman2019provably} & 0.360 (43\%) & 0.688 (47.2\%) & \textbf{0.910} (38.8\%)\\
\ourmethod & \textbf{0.391} (47.2\%) & \textbf{0.696} (47\%) & 0.894 (39.4\%)\\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> tables/table_short_svhn.tex <==
\begin{table}[t]
\caption{SVHN: clean accuracy and ACR of different models evaluated at the first 500 test images of SVHN with $\sigma=0.25$.}
\label{table_short_svhn}
\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc} 
\begin{tabular}{lccccr}
\toprule
 Model & Accuracy & ACR\\
\midrule
SmoothAdv & 85.8\% & 0.560\\
MACER & 86.8\% & 0.549\\
\ourmethod & 86.6\% & \textbf{0.569}\\
\midrule
\EsbRs{-}SmoothAdv$\times$3 & 87.8\% & 0.578\\
\EsbRs{-}\ourmethod$\times$3 & 88.2\% & \textbf{0.582}\\
\EsbRs{-}\ourmethod$\times$1+MACER$\times$2 & 87.8\% & 0.559\\
\EsbRs{-}\ourmethod$\times$2+MACER$\times$1 & 88.6\% & 0.570\\
\EsbRs{-}\ourmethod$\times1$+SmoothAdv$\times2$ & 87.8\% & 0.577\\
\EsbRs{-}\ourmethod$\times2$+SmoothAdv$\times1$ & 87.6\% & \textbf{0.582}\\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\end{table}

==> tables/table_soft.tex <==
\begin{table}[ht]
\caption{Soft RS: soft certified radius and the number of images that has larger soft CR. The experiment is on the first 500 test images of Cifar-10 with $\sigma=0.25$. Note that the ACR is much smaller than that in \cref{table_cifar10} since soft-RS is applied.}
\label{table_soft}
\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc} 
\begin{tabular}{lcr}
\toprule
Model & Soft ACR & \# points with larger ACR\\
\midrule
\ourmethod1 & 0.273 & { 365}\\
\ourmethod2 & 0.265 & 135\\
Esb-\ourmethod$\times2$ & \textbf{0.279} & NA\\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\end{table}

==> tables/table_svhn_full.tex <==
\begin{table*}[t]
\caption{SVHN: clean accuracy and ACR of different models evaluated at the full test images of SVHN at $\sigma=0.25$.}
\label{table_svhn}
\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc} 
\begin{tabular}{lccccr}
\toprule
 $\sigma$ & Model & Accuracy & ACR & Training Time\\
\midrule
\multirow{9}{2em}{$0.25$}
%& \cite{cohen2019certified}  & 88.2\% & 0.497 & 1.24h\\
& SmoothAdv & 87.2\% & 0.566 & 11.4h\\
& MACER & 88.6\% & 0.552 & 48.5h\\
& \ourmethod & 88.1\% & \textbf{0.571} & 11.4h\\
\cmidrule{2-5}
& \EsbRs{-}SmoothAdv$\times$3 & 88.3\% & 0.587 & NA\\
& \EsbRs{-}\ourmethod$\times$3 & 88.4\% & \textbf{0.588} & NA\\
& \EsbRs{-}\ourmethod$\times$1+MACER$\times$2 &  89.1\% & 0.565 & NA\\
& \EsbRs{-}\ourmethod$\times$2+MACER$\times$1 & 89.0\% & 0.573 & NA\\
& \EsbRs{-}\ourmethod$\times1$+SmoothAdv$\times2$ & 88.3\% & 0.587 & NA\\
& \EsbRs{-}\ourmethod$\times2$+SmoothAdv$\times1$ & 88.5\% & 0.587 & NA\\
% \midrule
% \multirow{9}{2em}{$0.50$}
% %& \cite{cohen2019certified} & 68.8\% & 0.495 & 1.24h\\
% & SmoothAdv & 71.2\% & 0.552 & 11.4h\\
% & MACER & 58.4\% & 0.535 & 48.5h\\
% & \ourmethod & 67.8\% & \textbf{0.572} & 11.4h\\
% \cmidrule{2-5}
% & \EsbRs{-}SmoothAdv$\times$3 & 71.2\% & 0.573 & NA\\
% & \EsbRs{-}\ourmethod$\times$3 & 70.4\% & \textbf{0.588} & NA\\
% & \EsbRs{-}\ourmethod$\times$1+MACER$\times$2 & 62.8\% & 0.551 & NA\\
% & \EsbRs{-}\ourmethod$\times$2+MACER$\times$1 & 66.0\% & 0.564 & NA\\
% & \EsbRs{-}\ourmethod$\times1$+SmoothAdv$\times2$ & 71.8\% & 0.577 & NA\\
% & \EsbRs{-}\ourmethod$\times2$+SmoothAdv$\times1$ & 71.2\% & 0.583 & NA\\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\end{table*}

==> tables/table_univ_config.tex <==
\begin{table}[ht]
\caption{Universal configuration: clean accuracy and ACR evaluated at the first 500 test images of Cifar10. We choose $T=m=2$ across all SmoothAdv and \ourmethod models. For comparison, we also report the results from MACER.}
\label{table_univ_config}
\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc} 
\begin{tabular}{lcccccr}
\toprule
 $\sigma$ & Model & Accuracy & ACR & $\epsilon$ & Time\\
\midrule
\multirow{3}{2em}{$0.25$}
& MACER & 79.4\% & \textbf{0.518} & NA & 32.8h\\
& SmoothAdv & 71\% & 0.517 & 1.0 & 3.9h\\
& \ourmethod & 70.4\% & 0.516 & 1.0 & 3.9h\\
\midrule
\multirow{3}{2em}{$0.50$}
& MACER & 63.4\% & 0.682 & NA & 32.8h\\
& SmoothAdv & 51.8\% & 0.714 & 2.0 & 3.9h\\
& \ourmethod & 52.8\% & \textbf{0.721} & 2.0 & 3.9h\\
\midrule
\multirow{3}{2em}{$1.00$}
& MACER & 42.4\% & 0.768 & NA & 32.8h\\
& SmoothAdv & 43.4\% & 0.756 & 2.0 & 3.9h\\
& \ourmethod & 44.4\% & \textbf{0.781} & 2.0 & 3.9h\\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\end{table}

